Learning-based feedforward augmentation for steady state rejection of residual dynamics on a nanometer-accurate planar actuator system

Growing demands in the semiconductor industry result in the need for enhanced performance of lithographic equipment. However, position tracking accuracy of high precision mechatronics is often limited by the presence of disturbance sources, which originate from unmodelled or unforeseen deterministic environmental effects. To negate the effects of these disturbances, a learning based feedforward controller is employed, where the underlying control policy is estimated from experimental data based on Gaussian Process regression. The proposed approach exploits the property of including prior knowledge on the expected steady state behaviour of residual dynamics in terms of kernel selection. Corresponding hyper-parameters are optimized using the maximization of the marginalized likelihood. Consequently, the learned function is employed as augmentation of the currently employed rigid body feedforward controller. The effectiveness of the augmentation is experimentally validated on a magnetically levitated planar motor stage. The results of this paper demonstrate the benefits and possibilities of machine-learning based approaches for compensation of static effects, which originate from residual dynamics, such that position tracking performance for moving-magnet planar motor actuators is improved.

==> Chapters/NAPAS_Prototype.tex <==
\label{NAPASProto}
\subsection{System Overview}
\hspace*{2mm} The Nanometer Accurate Planar Actuator System (NAPAS prototype), which is depicted in Figure \ref{NAPAS}, consists of three main components, which are not physically connected to each other: the stator base ($\mathcal{C}$), the translator ($\mathcal{T}$) and the metrology frame ($\mathcal{M}$). The stator base is a double layer coil array, consisting of 160 coils of which 40 coils are enabled using 40 power converters at a single time instant, dependent on the relative position of the translator. Proper actuation of the coils offers the means of both stabilization and propulsion of the magnet plate in 6 Degrees of Freedom (DOFs). The metrology frame, which is rested on air mounts to suppress effects of floor disturbances, is used as a global reference frame, such that position tracking accuracy can be evaluated. On the metrology frame, 9 laser interferometers (LIFMs) are mounted to measure the relative displacement of the translator respectively. Additionally, two sets of eddy current sensors (ECS) are mounted as auxiliary measurement systems, where one set of ECS is used for initialization of the NAPAS system
and the second set of ECS is used to capture the displacements between the stator base and the metrology frame ($\mathcal{C}$-$\mathcal{M}$). In order to relate the coordinate frames to each other, rigid body coordinate frame transformations are applied, see \cite{Murray-book}. 

\begin{figure}[h]
\begin{center}
\includegraphics[width=\linewidth]{Figures/ML paper 2D.pdf}
\end{center}
\caption{Schematic representation of the NAPAS setup, with a) six ECS ($\mathcal{C}$-$\mathcal{T}$), which are used for initialization of the system. b) IFM sensors, which measure the relative position of the translator with respect to the metrology frame ($\mathcal{T}$-$\mathcal{M}$). c) Six stator-to-metrology ECs ($\mathcal{C}$-$\mathcal{M}$), which are used to measure the displacements between the stator and the metrology frame. $\bar{x}_\mathcal{M}$, $\bar{y}_\mathcal{M}$ and $\bar{z}_\mathcal{M}$ denote the coordinate frame with respect to the metrology frame.}
\label{NAPAS}
\end{figure}

\noindent
\hspace*{2mm} The dynamic behaviour of the planar motor is governed by both electromagnetic and mechanical phenomena. The electromagnetic interaction describes the relation between the input currents in the coils and the resulting magnet force distribution on the magnet plate of the translator. The mechanical model describes the relation between the aforementioned force distribution and the resulting motion of the translator. The relative displacement of the translator with respect to the metrology frame is captured by the LIFMs.


\subsection{Electromagnetic interaction}

\hspace*{2mm} The actuation of the electromagnetically-levitated planar motor is realized by 40 power amplifiers, which independently control the current supplied to the corresponding 40 active coils. The relation between the supplied currents, $\boldsymbol{i} \in \mathbb{R}^{40}$, and the resulting force vector, is described by the Lorentz force principle \citep{173Rovers}. Under the rigid-body assumption, the force distribution, exerted on the magnet plate, is equivalently described as a force and torque vector around the center of mass \citep{Murray-book}. Since the position of the plate is evaluated with respect to the metrology frame, $\mathcal{M}$, it is convenient to define the force/torque vector with respect to the same frame.  This force/torque vector is defined as
\begin{align}
\boldsymbol{W}_{\mathcal{M}} = \begin{bmatrix}
F_x & F_y & F_z & \tau_x & \tau_y & \tau_z
\end{bmatrix}^\top,
\end{align}
%
where $F_x$ and $\tau_x$ are the force and torque acting on the $x$ axis (similarly for the other axes), expressed on the metrology frame. Then, the electromagnetic interaction is defined by
%
\begin{align}
\boldsymbol{W} _{\mathcal{M}}
&= 
R^{\mathcal{M}}_{\mathcal{C}} 
M^{\mathrm{r}} \left( \boldsymbol{q}^{\mathcal{C}}_{\mathcal{T}} \right) \boldsymbol{i},
\label{eq:rigidbodyEM}
\end{align}
%
%
where $M^{\mathrm{r}}: \mathbb{R}^6 \mapsto \mathbb{R}^{n_{\mathrm{r}} \times 40}$ is a position dependent matrix, which depends on the relative position between the coil and the translator frame (magnet plate), which is denoted as $\boldsymbol{q}^{\mathcal{C}}_{\mathcal{T}}$. Moreover, since the force/torque vector is expressed with respect to the coil frame, the rotation matrix $R^{\mathcal{M}}_{\mathcal{C}}$ transforms the force and torque vector to the metrology coordinate frame.

\subsection{Mechanical system}

\hspace*{2mm} Under rigid-body assumption, the dynamics of the translator are derived using Euler-Lagrange modelling strategies. In the Euler-Lagrange approach, kinetic co-energy $\mathcal{T}^*(q_\mathcal{T}^\mathcal{M})$ and potential energy $\mathcal{V}(q_\mathcal{T}^\mathcal{M})$ of the translator are used for the construction of the kinematics of the translator \cite{184Jeltsema}. Equation \ref{EulerLagrange} illustrates the Euler-Lagrange equation, where the Lagrangian $\mathcal{L}(q_\mathcal{T}^\mathcal{M},\dot{q}_\mathcal{T}^\mathcal{M}) = \mathcal{T}^*(q_\mathcal{T}^\mathcal{M})-\mathcal{V}(q_\mathcal{T}^\mathcal{M})$ and $W_{gen}$ represents the generalized forces that act on the generalized coordinates $q_\mathcal{T}^\mathcal{M}$.


\begin{equation}
\frac{d}{dt} \frac{\partial \mathcal{L}(q_\mathcal{T}^\mathcal{M},\dot{q}_\mathcal{T}^\mathcal{M})}{\partial \dot{q}_\mathcal{T}^\mathcal{M}} - \frac{\partial \mathcal{L} (q_\mathcal{T}^\mathcal{M},\dot{q}_\mathcal{T}^\mathcal{M})}{\partial q_\mathcal{T}^\mathcal{M}} = W_{gen}
\label{EulerLagrange}
\end{equation}

%\noindent
%Equation \ref{KinCoEnergy} illustrates the kinetic co-energy in metrology coordinates, where $\rho$ denotes the density of a infinitesimal mass at a distance $r_\mathcal{T}$ from the origin of the coordinate frame $\mathcal{T}$, expressed in translator coordinates.

%\begin{equation}
%\mathcal{T}^* (q_\mathcal{T}^\mathcal{M}) = \frac{1}{2} \int_{V_\mathcal{M}} \rho(r_\mathcal{M}) \begin{pmatrix}
%\big | \big | \dot{R}_\mathcal{T}^\mathcal{M} r_\mathcal{T} \big | \big |_2^2 + 2{r_\mathcal{T}}^\top {\dot{R}_\mathcal{T}^\mathcal{M^\top}} \dot{p}_\mathcal{T}^\mathcal{M} + \big | \big | \dot{p}_\mathcal{T}^\mathcal{M} \big | \big |_2^2 
%\end{pmatrix}dV
%\label{KinCoEnergy}
%\end{equation}

%\noindent
%The potential energy of the translator is given by equation \ref{PotEnergy} under the assumption that the metrology frame corresponds to zero potential level.

%\begin{equation}
%\mathcal{V}(q_\mathcal{T}^\mathcal{M}) = m\cdot g\cdot z_\mathcal{T}^\mathcal{M}
%\label{PotEnergy}
%\end{equation}

\noindent
The established Euler-Lagrange equation, illustrated in equation \ref{EulerLagrange}, is rewritten as \cite{Spong}, which is illustrated by equation \ref{eq:MechanicalEquation}, where $W_{gen} = J^\top(q_\mathcal{T}^\mathcal{M})R_\mathcal{T}^\mathcal{M^\top} (W_\mathcal{M} - G_\mathcal{M})$ as shown in \cite{Proimadis-phd}, where $W_\mathcal{M}$ is constructed using equation \ref{eq:rigidbodyEM} and $G_\mathcal{M}$ denotes a vector containing the gravity compensation of the magnet plate.
\begin{equation}
M(q_\mathcal{T}^\mathcal{M})\ddot{q}_\mathcal{T}^\mathcal{M} + C(q_\mathcal{T}^\mathcal{M},\dot{q}_\mathcal{T}^\mathcal{M})\dot{q}_\mathcal{T}^\mathcal{M} = J^\top(q_\mathcal{T}^\mathcal{M})R_\mathcal{T}^\mathcal{M^\top} (W_\mathcal{M} - G_\mathcal{M})
\label{eq:MechanicalEquation}
\end{equation} 

\noindent
In lithographic equipment, rotational axes are steered to zero. Consequently, rotation angles are neglectable during application as shown by \cite{176Butler}. Therefore, a small angle approximation is applied to simplify the dynamics of the translator. The state space representation of the corresponding system is expressed by equation  \ref{eq:SSrepresentationDynamics}.
%, where $B_r = diag(\frac{1}{m},\frac{1}{m},\frac{1}{m},\frac{1}{\mathcal{I}_x},\frac{1}{\mathcal{I}_y},\frac{1}{\mathcal{I}_z})$.

\begin{equation}
\begin{bmatrix}
\dot{q}_\mathcal{T}^\mathcal{M} \\ 
\ddot{q}_\mathcal{T}^\mathcal{M}
\end{bmatrix} = 
\begin{bmatrix}
0 & I \\ 0 & 0
\end{bmatrix}
\begin{bmatrix}
q_\mathcal{T}^\mathcal{M} \\ \dot{q}_\mathcal{T}^\mathcal{M}
\end{bmatrix} + \begin{bmatrix}0 \\ B_r \end{bmatrix}
(W_\mathcal{M}-G_\mathcal{M})
\label{eq:SSrepresentationDynamics}
\end{equation}

\subsection{Control principles}
\hspace*{2mm} The magnetically levitated planar motor system is a coupled, position dependent MIMO system. In order to apply SISO control strategies for the design of a feedback controller, the system is rigid body decoupled \cite{190Steinbuch}, such that the equivalent plant, seen by the feedback controller, is approximately diagonal up until the desired bandwidth \cite{185Wal}. For construction of a feedback controller, a combination of a PID controller and a low-pass filter is considered for all six physical axes. Additionally, a diagonal mass feedforward is employed to the control system to further enhance position tracking performance.
The corresponding feedforward force is dependent on the acceleration profile that is being applied to the system, which is designed using a fourth order reference trajectory generator \cite{208Lambrechts}. As mentioned in section \ref{Introduction}, the NAPAS system is subject to various disturbance sources, which originate from unforeseen and deterministic environmental effects. Compensation of these disturbances in terms of feedforward control requires a disturbance model. The construction of the disturbance model is presented in section \ref{ch:Gplearning}.


%Since the translator is a complex dynamical system, FEM software is used to derive the equations of motion of the translator $\Sigma_p(\rho(t),t)$. Equation \ref{GeneralizedDynamicEquation} illustrates the generalized dynamics, where $M$, $D$ and $K$ are the real symmetric mass, damping and stiffness matrices with dimension $p\times p$ and $F_\mathcal{M}^M(t) \in \mathbb{R}^{l}$. 


%\begin{equation}
%M\ddot{x}(t) + D\dot{x}(t)+Kx(t) = GF_\mathcal{M}^M(t)
%\label{GeneralizedDynamicEquation}
%\end{equation}

%\noindent
%To internally decouple the dynamics, the system is represented in modal form. This is achieved by performing a basis transformation using the eigenvector $\Phi \in \mathbb{R}^{p\times p}$, which is obtained by solving the characteristic dynamical equation $K\Phi = M\Phi\Lambda$. The modal system representation is illustrated in equation \ref{ModalSystem}, where $x(t) = \Phi q(t)$ and the eigenvector matrix $\Phi$ is mass normalized, implying $\Phi^\top M \Phi = I$. $Z \in \mathbb{R}^{p\times p}$ denotes a diagonal matrix containing the modal damping parameters and $\Omega \in \mathbb{R}^{p \times p}$ denotes a diagonal matrix containing the eigenfrequencies of the dynamical system in radians per second respectively.
%\begin{equation}
%\ddot{q}(t) + 2Z\Omega\dot{q}(t)+\Omega^2 q(t) = \Phi^\top GF_\mathcal{M}^M(t)
%\label{ModalSystem}
%\end{equation}

%\noindent To interconnect the mechanical system of the translator with $\Sigma_{EI}(\rho(t),t)$ and $\Sigma_\mathcal{M}(\rho(t))$, the mechanical translator system is represented in state space form as illustrated in equation \ref{ModalStateSpace}, where $\bar{q} = \begin{bmatrix}
%q(t) & \dot{q}(t)
%\end{bmatrix}^\top$ and $x_{IFM}(t) \in \mathbb{R}^9$. $\Phi_s(\rho(t))$ denotes the mapping of the appropriate modal masses to the output $x_{IFM}(t)$.

%\begin{equation}
%\Sigma_p(\rho(t),t) := 
%\begin{cases}
%\begin{split}
%\dot{\bar{q}}(t) &= \begin{bmatrix}
%0 & I \\ -2Z\Omega & -\Omega^2
%\end{bmatrix}\bar{q}(t) + 
%\begin{bmatrix}
%0 \\ \Phi^\top G
%\end{bmatrix}
%F_\mathcal{M}^M(t)
%\\
%x_{IFM}(t) &= \begin{bmatrix}
%\Phi_s(\rho(t)) & 0 
%\end{bmatrix}\bar{q}(t) 
%\end{split}
%\end{cases}
%\label{ModalStateSpace}
%\end{equation}
